QuantumDNA: A Python Package for Analyzing Quantum Charge Dynamics in DNA and Exploring Its Biological Relevance

The study of DNA charge dynamics is a highly interdisciplinary field that bridges physics, chemistry, biology, and medicine, and plays a critical role in processes such as DNA damage detection, protein-DNA interactions, and DNA-based nanotechnology. However, despite significant advances in each of these areas, knowledge often remains inaccessible to other scientific communities, limiting the broader impact of advances across disciplines. To bridge this gap, we present QuantumDNA, an open-source Python package for simulating DNA charge transfer (CT) and excited states using quantum-physical methods. QuantumDNA combines an efficient Linear Combination of Atomic Orbitals (LCAO) approach with tight-binding (TB) models, incorporating open quantum systems techniques to account for environmental effects. This approach allows rapid yet accurate analysis of large DNA ensembles, enabling statistical studies of genetic and epigenetic phenomena. To ensure accessibility, the package features a graphical user interface (GUI), making it suitable for researchers across disciplines.

==> chapters/0_program_summary.tex <==
% \onecolumn

{\bf PROGRAM SUMMARY}\\
\begin{small}
\noindent
{\em Program Title:} QuantumDNA \\
{\em CPC Library link to program files:}\\ (to be added by Technical Editor) \\
{\em Developer's repository link:}\\ https://github.com/dehe1011/QuantumDNA \\
{\em Code Ocean capsule:} (to be added by Technical Editor) \\
{\em Licensing provisions:} BSD 3-clause \\
{\em Programming language:} Python \\

{\em Nature of the Problem:} Despite more than 60 years of research, DNA charge dynamics remains a fragmented field, with theoretical and computational advances often inaccessible across disciplines. A standardized platform that integrates methods from computational physics, quantum chemistry, and molecular biology is essential to promote a comprehensive understanding and facilitate interdisciplinary collaboration.

{\em Solution Method:} QuantumDNA is an open-source package that unifies different computational approaches to DNA charge transport and excited states. It integrates LCAO and TB models with open quantum systems methods to simulate charge dynamics while accounting for environmental effects. Unlike computationally expensive \emph{ab initio} methods, QuantumDNA allows efficient analysis of large DNA sequence ensembles, making it particularly valuable for statistical investigations in genetics and epigenetics.

{\em Additional comments:} QuantumDNA features a GUI, making it accessible to researchers with limited computer experience. The package includes comprehensive documentation, tutorial Jupyter notebooks, and a dedicated documentation website to facilitate learning and implementation. The package also supports CPU parallel computing, enabling efficient analysis of large DNA datasets.

% Bibliography for Program Summary
% begin{thebibliography}{0}
% \bibitem{TB_models}
% T. Chakraboty, Charge Migration in DNA: Perspectives from Physics, Chemistry, and Biology, Springer, Berlin, Heidelberg, 2007.
% \end{thebibliography}

\end{small}

% \twocolumn

==> chapters/remainings.tex <==
. There is fast long-range CT in DNA 
. CT is sensitive to perturbations in the base stacking
. CT happens mainly through pi-orbitals of stacked DNA nucleobases (not sugar-phosphate backbone)
. The mechanism of CT is not fully understood. Combination of superexchange (quantum tunnelling), classical thermal hopping, gating by low frequency fluctuations of environmental degrees of freedom (nuclei, backbone)

. DNA base stacking is altered by: TATA-box-binding protein (kinking leads to worse stacking), cytosine methylation (increased stiffness leads to better stacking)
. CT might be used as fast and efficient scanning and signaling mechanism in the cell
. CT might be used for DNA repair and gene regulation (because of changes in the stacking) by proteins containing redox active iron-sulfur clusters [4Fe4S]

. Simulation and Modelling: ab initio atomistic calculations are limited to small sequences (up to four bases) close to equilibrium 


From a quantum physics point of view DNA charge dynamics at ambient cellular conditions can be described as open quantum system, i.e., as system in contact with a thermal reservoir. The separation between system and bath typically used is reflected in the package structure of QuantumDNA.  

% ----------------------------------------------
% Remainings
% ----------------------------------------------

% Dephasing Models and Equilibrium States
The dephasing models are feasible for simulations in the short time regime, since they do not equilibrate to the canonical thermal state in the long time regime. As shown in \cite{Abbott2020}, they can give good qualitative agreement with the HEOM dynamics for an appropriate choice of dephasing rate. The local dephasing model reaches the fully mixed state ($\lim_{t\to\infty}\rho(t) = \mathbb{I}/N$) for long times, meaning that coherences die out completely. In contrast, coherences survive in the global dephasing model, as shown in \cite{Rossini2024} where the equilibrium density matrix reflects the eigenstate decomposition of the initial state $\rho_0$:

\begin{align}
    \lim_{t\to\infty} \rho(t) &= \sum_{\alpha,\beta\in\Lambda}\sum_{i=1}^N \bra{\Psi_i}\rho_0\ket{\Psi_i}\, c_{\alpha i} c_{\beta i}^* \ket{\alpha}\bra{\beta}.
\end{align} 

% Thermalizing Models
Thermalizing models are based on the Redfield rate $k(\omega)$, which is derived from the Fourier transform of the bath correlation function. At body temperature, the Bose-Einstein distribution $n(\omega)$ for the environmental degrees of freedom remains relatively small, causing the rate to approximate the spectral density and become nearly temperature independent. QuantumDNA implements two types of spectral densities-Ohmic and Debye-both of which increase linearly with frequency up to a high frequency cutoff. As a result, Redfield rates are reduced at high frequencies (corresponding to large energy separations) due to the high-frequency cutoff of the spectral density.   

\begin{align}
    k(\omega) = 2\pi \left[ J(\omega)(1+n(\omega))+ J(-\omega)n(-\omega) \right]
\end{align}

When the TB sites are far apart, the transfer energies become infinitesimally weak, causing the eigenstates to closely resemble the local states. In such cases, the global thermalizing model inaccurately predicts population transfer between TB sites that does not actually occur, revealing its limitations under weak coupling conditions. In contrast, the local thermalizing model avoids this unphysical population transfer, as the product $c^*_{\alpha,j}c_{\alpha,i}$ approaches zero \cite{Abbott2020}.

% Löwdin proton tunnelling
The integration of quantum physical principles has proven valuable in advancing our understanding of biological processes. For example, Löwdin's pioneering work demonstrated that classically forbidden proton tunneling through energy barriers could lead to DNA point mutations, shedding light on a fundamental mechanism of genetics \cite{Löwdin1963}.
